An App for the Discovery of Properties of Poncelet Triangles

We describe a newly-developed, free, browser-based application, for the interactive exploration of the dynamic geometry of Poncelet families of triangles. The main focus is on responsive display of the beauteous loci of centers of such families, refreshing them smoothly upon any changes in simulation parameters. The app informs the user when curves swept are conics and reports if certain metric quantities are conserved. Live simulations can be easily shared via a URL. A list of more than 400 pre-made experiments is included which can be regarded as conjectures and/or exercises. Millions of experiment combinations are possible.

==> 015_example.tex <==
\section{An example of a discovery workflow}

\begin{itemize}

\item[(a)] Poncelet triangles family inscribed in parabola, circumscribing focus-centered circle: locus of $X_4$ is a line. (needs proof)

\item[(b)] intouch triangles of (a) has stationary $X_1$ and fixed inradius $r$. since inscribed in fixed circle, it is a bicentric N=3 family. One notices the incircle passes thru $X_3$, i.e., $d=|OI|=r$.Since $d = \sqrt(R(R-2r))$, setting $d=r$ implies $r/R = \sqrt(2)-1 = r_0$.

\item[(c)] this implies (a) are tangential triangles to bicentrics N=3. If $r<r_0$ (resp. $r>r_0$), the locus of tangential vertices is an ellipse (resp. hyperbola). 

\item[(d)] $X_4$ of tangential is $X_{155}$ of reference (bicentrics). With $r<r_0$ (resp. $r>r_0$), locus of these is either ellipse, or hyperbola, with a parabola achieved when $r=r_0$.

\item[(e)] a well-known fact is that the orthic triangle is homothetic to the tangential. observe that if $r<r_0$ (resp. $r>r_0$), locus of $X_1$ of orthic is a circle corresponding to $X_4$ of reference, (resp. the union of two circles: tracking $X_4$ of reference while the latter is acute, and railing itself to the circumcircle -- the obtuse vertex -- while the latter is obtuse).

\item[(f)] also observe that while the bicentric triangle is acute, $L_{ort}/L$ is conserved. A well-known fact is that if reference is acute, $L_{ort}=2R\sum\sin(2\theta_i)=2R\sum{\sin\theta_i \cos\theta_i}$. Since R is constant over bicentrics, this implies that for acute bicentrics, $\sum(2\theta_i)/L$ must be conserved.

\item[(g)] since over N=3 Poncelet interscribed in ellipse and concentric incircle, R is conserved, then this family must also conserve $\sum(2\theta_i)/L$ while the triangles are acute.

\item[(h)] observe that for either bicentric or (f) N-gons, $\sum(2\theta_i)/L$ is conserved. (no proof)

\item[(i)] for any family of N-gons with a fixed incircle of radius r, $A=(1/2) r L$. Therefore $A/L$ is constant over such a family. Corollary: for both bicentrics and (f) N-gons, $\sum(2\theta_i)/A$ is also conserved. 
\end{itemize}

==> 030_triangle_families.tex <==
\section{Triangle Families}
\label{sec:families}

Experiments quickly identify special euclidean quantities each family conserves. For example, both the inellipse and homothetic families conserves the sum of their {\em squared sidelengths}. While the former conserves the product of internal angle cosines, the latter conserves the sum of internal angle cotangents! Compare these with the confocal family, whose perimeter (i.e., the sum of sidelengths), and {\em sum} of its internal angle cosines are conserved


==> 100_conclusion.tex <==
\begin{table}[H]
\scriptsize
\begin{tabular}{|c|l|l|l|}
\hline
\href{youtu.be}{PL\#} & Title & Narrated \\
\hline
\href{youtu.be}{01} & 
\makecell[lt]{xxx} & no \\
\hline
\end{tabular}
\caption{Playlist of videos. Column ``PL\#'' indicates the entry within the playlist.}
\label{tab:videos}
\end{table}

==> refs_rgk_media.tex <==
@MISC{impa2019,
   author = {Dan Reznik and Ronaldo Garcia and Jair Koiller},
   title = {Adventures with Triangles and Billiards},
   url={impa.br/en_US/eventos-do-impa/eventos-2019/ 32o-coloquio-brasileiro-de-matematica},
   address={Rio de Janeiro},
   institution = {Instituto Nacional de    Matemática Pura e Aplicada (IMPA)},
   day={31},
   month={7},
   year={2019},
}

@MISC{impa2019_video,
   author = {Dan Reznik and Ronaldo Garcia and Jair Koiller},
   title = {Adventures with Triangles and Billiards},
   url={youtu.be/t872mftaI2g},
   publisher={YouTube},
   day={15},
   month={8},
   year={2019},
}

@MISC{reznik_web,
   author = {Dan Reznik and Ronaldo Garcia and Jair Koiller},
   title={New Properties of Triangular Orbits in Elliptic Billiards},
   url={dan-reznik.github.io/Elliptical-Billiards-Triangular-Orbits/},
   year={2019}
}

@MISC{reznik_media,
   author = {Dan Reznik and Ronaldo Garcia and Jair Koiller},
   title={Media for Elliptic Billards and Family of Orbits},
   url={dan-reznik.github.io/Elliptical-Billiards-Triangular-Orbits/videos.html},
   year={2019}
}

@MISC{reznik_loci,
   author = {Dan Reznik},
   title={Triangular Orbits in Elliptic Billards: Loci of Points {X}(1)~{X}(100)},
   url={dan-reznik.github.io/Elliptical-Billiards-Triangular-Orbits/loci_6tri.html},
   year={2019}
}

@MISC{dsr_vid11incenter,
  author={Dan Reznik},
  title={Triangular Orbits in Elliptic Billiards: Locus of the Incenter is an Ellipse},
  year={2011},
  url={youtu.be/9xU6T7hQMzs},
  publisher={YouTube}
}

@MISC{dsr_vid11e,
  author={Dan Reznik},
  title={Locus of the incircle touchpoints is a higher-order curve},
  year={2011},
  url={youtu.be/9xU6T7hQMzs},
  publisher={YouTube}
}

@MISC{dsr_applet11a,
  author={Dan Reznik},
  title={"Dynamic Billiards in Ellipse"},
  url={demonstrations.wolfram.com/DynamicBilliardsInEllipse/},
  publisher={Wolfram Demonstrations Project},
  year={2011}
}

@MISC{playlist2020-deltoid,
author={Dan Reznik},
  title={{YouTube} Playlist for Constant-Area Deltoid},
  year={2020},
  publisher={YouTube},
  url={bit.ly/3gqfIRm}
}

@MISC{dsr_main_videos_2019,
  author={Dan Reznik},
  title={New Properties of Polygonal Orbits in Elliptic Billiards: Main Videos},
  year={2019},
  url={bit.ly/2k5GXbB},
  publisher={YouTube}
}

@MISC{dsr_playlist_2020,
  author={Dan Reznik},
  title={Playlist for {``Loci of Triangular Orbits in an Elliptic Billiard''}},
  year={2020},
  url={bit.ly/3072LV3},
  publisher={YouTube}
}

@MISC{dsr_playlist_2020_proofs,
  author={Dan Reznik},
  title={Playlist for {``New Properties of Triangular Orbits in an Elliptic Billiard''}},
  year={2020},
  url={bit.ly/379mk1I},
  publisher={YouTube}
}

@MISC{dsr_playlist_2020_polygons,
  author={Dan Reznik},
  title={Playlist for {``Invariants of N-Periodics in the Elliptic Billiard''}},
  year={2020},
  url={bit.ly/2xeVGYw},
  publisher={YouTube}
}

@MISC{dsr_playlist_2020_invariants,
  author={Dan Reznik},
  title={Playlist for {``Invariants of N-Periodic Trajectories in Elliptic Billiards''}},
  year={2020},
  url={bit.ly/3aNqgqU},
  publisher={YouTube}
}


@MISC{dsr_locus_gallery_2019,
  author={Dan Reznik},
  title={Triangular Orbits in Elliptic Billards: Loci of Points {X(1)~X(100)}},
  year={2019},
  url={dan-reznik.github.io/Elliptical-Billiards-Triangular-Orbits/loci_6tri.html},
  publisher={GitHub}
}

@MISC{dsr_applet_x12345,
author={Dan Reznik},
  title={Applet Showing the Locus of Several Triangular Centers},
  year={2019},
  publisher={P5.js},
  url={editor.p5js.org/dreznik/full/i1Lin7lt7}
}

@MISC{darlan2020-app,
author={Iverton Darlan and Dan Reznik},
title={Loci of Ellipse-Mounted Triangle Centers},
year={2020},
url={dan-reznik.github.io/ellipse-mounted-triangles/}
}

@MISC{sundrop2016,
author={Sundrop Farms},
title={February 2016 Update},
howpublished={{YouTube}},
year={2016},
url={https://youtu.be/rRNy89j6wMc}
}

@MISC{esolar2017,
author={General Electric},
title={{eSolar} Concentrated Solar plants},
howpublished={{YouTube}},
year={2017},
url={https://youtu.be/ADbUsuNeRQE}
}

@MISC{garcia2021-ellipses-web,
author={Ronaldo Garcia and Dan Reznik and Jair Koiller},
  title={Companion Website to ``Loci of 3-periodics in an Elliptic Billiard: Why so many ellipses?''},
  month={1},
  year={2021},
  howpublished={{GitHub Pages}},
  url={dan-reznik.github.io/why-so-many-ellipses/}
}

@MISC{reznik2021-observable-media,
author={Dan Reznik},
  title={Experimental {P}oncelet Media Assets},
  month={5},
  year={2021},
  howpublished={{Observable}},
  url={https://observablehq.com/@dan-reznik/poncelet-media-assets}
}

@MISC{reznik2021-observable-poncelet-closure,
author={Dan Reznik},
  title={{P}oncelet's Closure Theorem},
  month={5},
  year={2021},
  howpublished={{Observable}},
  url={https://observablehq.com/@dan-reznik/poncelet-iteration}
}

@MISC{reznik2021-observable-jacobi-elliptic-fns,
author={Dan Reznik},
  title={Jacobi's complete integral of first kind and elliptic functions},
  month={5},
  year={2021},
  howpublished={{Observable}},
  url={https://observablehq.com/@dan-reznik/jacobi-elliptic-functions}
}

@MISC{reznik2021-observable-spatiotemporal,
author={Claudio Esperança and Ronaldo Garcia and Dan Reznik},
  title={Elliptic Billiard 3-Periodics & Spatio-Temporal Visualization},
  month={5},
  year={2021},
  howpublished={{Observable}},
  url={https://observablehq.com/@dan-reznik/elliptic-billiard-triangle}
}

@misc{reznik2021-artful,
author={Dan Reznik},
Title={Artful Loci of Triangles in Ellipses},
year={2021},
howepublished={{Google Slides}},
url={bit.ly/34sO8Px}
}

@MISC{reznik2021-locus-app-tutorial,
title={Locus App Tutorial: a Video Walkthrough},
author={Dan Reznik},
year={2021},
howpublished={{YouTube}},
url={https://bit.ly/3iCKHxn}
}
